Equilibrium and non-equilibrium properties of active matter systems

Active matter systems encompass both natural and artificially created systems consisting of numerous active particles. These particles actively consume energy to propel themselves or exert mechanical forces, leading to intricate behaviors and a diverse range of collective motions from flocking transition to motility-induced phase separation. The flocking transition refers to the spontaneous alignment and coordination of individuals in a group, resembling the cohesive motion observed in flocks of birds or schools of fish. On the other hand, motility-induced phase separation refers to the segregation of active particles into distinct regions based on their differing motility levels. In this presentation, I will talk about active matter systems, specifically focusing on the collective behavior and dynamics, including the influence of volume exclusion features, the impact of disorder in the media, and the behavior of self-propelled particles in off-lattice domains by introducing spin anisotropy. The objective is to understand how the collective behavior of self-propelled particles is affected by various system parameters, including thermal noise, self-propulsion velocity, external field strength, etc. I will furthermore show the phenomena such as jamming, kinetic arrest, motility-induced phase separation, coexisting phases, microphase separation, and phase transitions within the context of active matter models.

==> Overview/Overview.tex <==
\chapter*{Overview of Thesis\markboth{overview}{overview}}

~~~~~~This thesis is devoted to the study of active matter systems, specifically focusing on the collective behavior and dynamics of self-propelled particles. The research explores various aspects of active matter, including the influence of volume exclusion features, the impact of disorder in the media, and the behavior of self-propelled particles in off-lattice domains by introducing spin anisotropy. The thesis aims to understand how volume exclusion, disorder, and system parameters such as temperature, self-propulsion velocity, and alignment parameters affect the collective behavior of self-propelled particles. It investigates phenomena such as jamming, kinetic arrest, motility-induced phase separation, coexisting phases, microphase separation, and phase transitions within the context of active matter models, particularly the active Potts model. Overall, the thesis contributes to the broader understanding of active matter physics and sheds light on the intriguing and diverse behavior of self-propelled particles in different scenarios and environments. The thesis is organized as follows:\\

{\bf Chapter 1} of this thesis serves as the Introduction, providing a concise overview of active matter systems, self-propelled particles, and their collective behavior. It discusses the motivation for studying these systems in diverse fields and introduces the phenomenon of Motility-Induced Phase Separation (MIPS). Additionally, the chapter highlights limitations in the current literature concerning active matter and outlines the methodologies employed in the research. This chapter sets the groundwork for the subsequent chapters, guiding the reader through the exploration of active matter phenomena and the investigation of emergent behaviors in self-propelled particles. \\

In {\bf Chapter 2}, we present a comprehensive Monte Carlo study that showed a discretized flocking model that can control particle mobility and produce a variety of self-organized patterns. The results showed that particle speed, temperature, and density all impact the local flux of particles, with increasing speed and density leading to increased particle flow. However, increased temperature rapidly changes the particle state and reduces effective flow. Significant volume exclusion leads to suppressed flow and promotes a jammed state. Results showed that boosting volume exclusion or increasing particle density reduces mobility due to cluster formation and local jamming, while increased thermal fluctuations increase particle transport, but the system becomes effectively jammed at high activity. The model's frozen or jammed state is a robust feature that resembles real-world systems, such as animal groups, pedestrian traffic, and robot swarms, which cause high-density clogs that quickly arrest into a frozen state. It would be interesting to investigate whether physiologically relevant active matter can avoid self-clogging.\\

This {\bf Chapter 3} of the thesis explores the behavior of self-propelled particles (SPPs) in disordered media using the $q$-state active Potts model. Three scenarios are investigated, including a constant external field with a fixed direction, a constant field with a random orientation in $q=4$ directions, and a random distribution of bonds with probability $P_{bd}$ between lattice sites. By determining the critical temperature, $T_c$, and critical local field strength, $h_c$, for the coexistence of different phases, the study shows that dilute bonds break the symmetry of interactions, leading to complex collective behavior. The analysis reveals that bond dilution causes a loss of spatial correlation and a formation of a disordered phase at $P_{bd} = P_{bd}^* \approx 0.24\pm 0.02$ for a 2D square lattice, beyond which long-range order is not observed. These findings have implications for understanding the behavior of SPPs in disordered media and for the application of active matter particles in various fields. The study highlights the value of the $q$-state active Potts model in exploring the collective behavior of SPPs in disordered media and provides insights into the effects of dilute bonds on the system.\\

In {\bf Chapter 4}, we present an extensive Monte Carlo study that has revealed that the magnetic avalanches found in the Dy-Fe-Ga alloy are a manifestation of self-organized criticality. Experimentally and through simulation, we have shown that the magnetization jumps in the alloy are stochastic and follow a scale-invariant power law distribution. This power law distribution is a hallmark of self-organized criticality, which occurs when a complex system evolves towards criticality through local interactions. In the case of the Dy-Fe-Ga alloy, the local interaction is a magnetic correlation between the Dy and Fe atoms. Our study results are consistent with the predictions of the BTW sandpile model, one of the earliest models of self-organized criticality. The staircase-like feature in the magnetization isotherms observed both in experiment and simulation, is due to the frustration in the magnetic interaction between the Fe and Dy domains and the requirement of a sufficient external magnetic field to flip the domains.\\

In {\bf Chapter 5}, we conclude the thesis with a summary and general discussions of the investigations presented in the previous chapters.

\clearpage

